Toward Enhancing Vehicle Color Recognition in Adverse Conditions: A Dataset and Benchmark

Vehicle information recognition is crucial in various practical domains, particularly in criminal investigations. Vehicle Color Recognition (VCR) has garnered significant research interest because color is a visually distinguishable attribute of vehicles and is less affected by partial occlusion and changes in viewpoint. Despite the success of existing methods for this task, the relatively low complexity of the datasets used in the literature has been largely overlooked. This research addresses this gap by compiling a new dataset representing a more challenging VCR scenario. The images - sourced from six license plate recognition datasets - are categorized into eleven colors, and their annotations were validated using official vehicle registration information. We evaluate the performance of four deep learning models on a widely adopted dataset and our proposed dataset to establish a benchmark. The results demonstrate that our dataset poses greater difficulty for the tested models and highlights scenarios that require further exploration in VCR. Remarkably, nighttime scenes account for a significant portion of the errors made by the best-performing model. This research provides a foundation for future studies on VCR, while also offering valuable insights for the field of fine-grained vehicle classification.

==> zbibtex-copy.tex <==
@article{chawla2002smote,
    title={SMOTE: synthetic minority over-sampling technique},
    author={Chawla, Nitesh V and others},
    journal={Journal of artificial intelligence research},
    volume={16},
    pages={321--357},
    year={2002}
}

@article{chen2014vehicle,
  author={Chen, Pan and Bai, Xiang and Liu, Wenyu},
  journal={IEEE Transactions on Intelligent Transportation Systems}, 
  title={Vehicle Color Recognition on Urban Road by Feature Context}, 
  year={2014},
  volume={15},
  number={5},
  pages={2340-2346},
  keywords={Image color analysis;Vehicles;Histograms;Support vector machines;Videos;Image recognition;Colored noise;Color recognition;region of interest (ROI);vehicle;Color recognition;region of interest (ROI);vehicle},
  doi={10.1109/TITS.2014.2308897}}

@article{hu2015vehicle,
  author={Hu, Chuanping and Bai, Xiang and Qi, Li and Chen, Pan and Xue, Gengjian and Mei, Lin},
  journal={IEEE Transactions on Intelligent Transportation Systems}, 
  title={Vehicle Color Recognition With Spatial Pyramid Deep Learning}, 
  year={2015},
  volume={16},
  number={5},
  pages={2925-2934},
  keywords={Image color analysis;Vehicles;Feature extraction;Support vector machines;Training;Histograms;Computer architecture;Color recognition;deep learning;convolutional neural network (CNN);spatial pyramid (SP);intelligent transportation;Color recognition;deep learning;convolutional neural network (CNN);spatial pyramid (SP);intelligent transportation},
  doi={10.1109/TITS.2015.2430892}
}

@article{hsieh2015vehicle,
    author={Hsieh, Jun-Wei and Chen, Li-Chih and Chen, Sin-Yu and Chen, Duan-Yu and Alghyaline, Salah and Chiang, Hui-Fen},
    journal={IEEE Sensors Journal}, 
    title={Vehicle Color Classification Under Different Lighting Conditions Through Color Correction}, 
    year={2015},
    volume={15},
    number={2},
    pages={971-983},
    keywords={Image color analysis;Color;Cameras;Lighting;Feature extraction;Space vehicles;Vehicle color classification;color correction;SVM;vehicle window removal},
    doi={10.1109/JSEN.2014.2358079}}


@article{goncalves2016benchmark,
  title = {Benchmark for license plate character segmentation},
  author = {G. R. {Gon{\c{c}}alves} and da Silva, Sirlene Pio Gomes and Menotti, David and Schwartz, William Robson},
  year = {2016},
  journal = {Journal of Electronic Imaging},
  volume = {25},
  number = {5},
  pages = {053034},
  doi = {10.1117/1.JEI.25.5.053034},
}

@article{zhang2018vehicle,
    title = {Vehicle color recognition using Multiple-Layer Feature Representations of lightweight convolutional neural network},
    journal = {Signal Processing},
    volume = {147},
    pages = {146-153},
    year = {2018},
    issn = {0165-1684},
    doi = {https://doi.org/10.1016/j.sigpro.2018.01.021},
    author = {Qiang Zhang and Li Zhuo and Jiafeng Li and Jing Zhang and Hui Zhang and Xiaoguang Li},
    keywords = {Multiple-Layer Feature Representations, Lightweight convolutional neural network, Vehicle color recognition, Spatial Pyramid Matching}
}

@article{fu2018mcff,
    title = {MCFF-CNN: Multiscale comprehensive feature fusion convolutional neural network for vehicle color recognition based on residual learning},
    journal = {Neurocomputing},
    volume = {395},
    pages = {178-187},
    year = {2020},
    issn = {0925-2312},
    doi = {https://doi.org/10.1016/j.neucom.2018.02.111},
    author = {Huiyuan Fu and others},
    keywords = {Vehicle color recognition, Convolutional neural network, Residual learning, Video surveillance, Intelligent transportation system}
}

@article{zhuo2018high,
    author = {Li Zhuo and Qiang Zhang and Jiafeng Li and Jing Zhang and Xiaoguang Li and Hui Zhang},
    title = {{High-accuracy vehicle color recognition using hierarchical fine-tuning strategy for urban surveillance videos}},
    volume = {27},
    journal = {Journal of Electronic Imaging},
    number = {5},
    publisher = {SPIE},
    pages = {051203},
    keywords = {vehicle color recognition, convolutional neural networks, hierarchical fine-tuning strategy, quality assessment, Data modeling, Image quality, Surveillance, Video, Video surveillance, Lithium, Image classification, Fourier transforms, Image processing, Intelligence systems},
    year = {2018},
    doi = {10.1117/1.JEI.27.5.051203},
}

@article{shorten2019survey,
    title={A survey on image data augmentation for deep learning},
    author={Shorten, Connor and Khoshgoftaar, Taghi M},
    journal={Journal of big data},
    volume={6},
    number={1},
    pages={1--48},
    year={2019},
    publisher={Springer}
}


@article{oliveira2021vehicle,
  title = {{Vehicle-Rear}: A New Dataset to Explore Feature Fusion for Vehicle Identification Using Convolutional Neural Networks},
  author = {I. O. {Oliveira} and R. {Laroca} and D. {Menotti} and K. V. O. {Fonseca} and R. {Minetto}},
  year = {2021},
  journal = {IEEE Access},
  volume = {9},
  number = {},
  pages = {101065-101077},
  doi = {10.1109/ACCESS.2021.3097964},
  issn = {2169-3536}
}

@article{hu2023vehicle,
  title={Vehicle color recognition based on smooth modulation neural network with multi-scale feature fusion},
  author={Hu, Mingdi and Bai, Long and Fan, Jiulun and Zhao, Sirui and Chen, Enhong},
  journal={Frontiers of Computer Science},
  volume={17},
  number={3},
  pages={173321},
  year={2023},
  publisher={Springer}
}

@proceedings{Sibgrapi2024,
	Address = {Manaus, AM, Brazil},
	Booktitle = {SIBGRAPI},
	Month = {October},
	Publisher = {{IEEE}},
	Title = {Proceedings of the 35th SIBGRAPI Conference on Graphics, Patterns and Images (SIBGRAPI)},
	Year = {2024}
}

@inproceedings{baek2007vehicle,
    author="Baek, Nakhoon and others",
    editor="Huang, De-Shuang
    and Heutte, Laurent
    and Loog, Marco",
    title="Vehicle Color Classification Based on the Support Vector Machine Method",
    booktitle="Advanced Intelligent Computing Theories and Applications. With Aspects of Contemporary Intelligent Computing Techniques",
    year="2007",
    publisher="Springer Berlin Heidelberg",
    address="Berlin, Heidelberg",
    pages="1133--1139",
    isbn="978-3-540-74282-1"
}

@inproceedings{son2007convolution,
    author={Son, Jeong-Woo and Park, Seong-Bae and Kim, Ku-Jin},
    booktitle={Sixth International Conference on Advanced Language Processing and Web Information Technology (ALPIT 2007)}, 
    title={A Convolution Kernel Method for Color Recognition}, 
    year={2007},
    volume={},
    number={},
    pages={242-247},
    keywords={Convolution;Kernel;Information technology;Convolution KernelKernel methodsSVMsColor Recognition},
    doi={10.1109/ALPIT.2007.28}
}

@inproceedings{deng2009imagenet,
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Kai Li and Li Fei-Fei},
  booktitle={2009 IEEE Conference on Computer Vision and Pattern Recognition}, 
  title={ImageNet: A large-scale hierarchical image database}, 
  year={2009},
  volume={},
  number={},
  pages={248-255},
  keywords={Large-scale systems;Image databases;Explosions;Internet;Robustness;Information retrieval;Image retrieval;Multimedia databases;Ontologies;Spine},
  doi={10.1109/CVPR.2009.5206848}
}


@inproceedings{dule1010convenient,
    author = {Dule, Erida and G\"{o}kmen, Muhittin and Berato\u{g}lu, M. Sabur},
    title = {A convenient feature vector construction for vehicle color recognition},
    year = {2010},
    isbn = {9789604741953},
    publisher = {World Scientific and Engineering Academy and Society (WSEAS)},
    address = {Stevens Point, Wisconsin, USA},
    booktitle = {Proceedings of the 11th WSEAS International Conference on Nural Networks and 11th WSEAS International Conference on Evolutionary Computing and 11th WSEAS International Conference on Fuzzy Systems},
    pages = {250–255},
    numpages = {6},
    keywords = {vehicle color recognition, outdoor color, histogram, feature selection, color spaces, classification method, ROI selection},
    location = {Iasi, Romania},
    series = {NN'10/EC'10/FS'10}
}

@inproceedings{mendesjunior2011towards,
  title = {Towards an automatic vehicle access control system: License plate location},
  author = {P. R. {Mendes J\'{u}nior} and others},
  year = {2011},
  month = {Oct},
  booktitle = {IEEE International Conference on Systems, Man, and Cybernetics},
  volume = {},
  number = {},
  pages = {2916-2921},
  doi = {10.1109/ICSMC.2011.6084108},
  issn = {1062-922X}
}

@inproceedings{he2016residual,
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={2016 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={Deep Residual Learning for Image Recognition}, 
  year={2016},
  volume={},
  number={},
  pages={770-778},
  keywords={Training;Degradation;Complexity theory;Image recognition;Neural networks;Visualization;Image segmentation},
  doi={10.1109/CVPR.2016.90}
}

@inproceedings{redmon2016yolo,
    author = {Redmon, Joseph and Divvala, Santosh and Girshick, Ross and Farhadi, Ali},
    title = {You Only Look Once: Unified, Real-Time Object Detection},
    booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
    month = {June},
    year = {2016}
} 

@inproceedings{jeong2017homogeneity,
  author={Jeong, Yoosoo and Park, Kil Houm and Park, Daejin},
  booktitle={2017 IEEE International Conference on Imaging Systems and Techniques (IST)}, 
  title={Homogeneity patch search method for efficient vehicle color classification using front-of-vehicle image}, 
  year={2017},
  volume={},
  number={},
  pages={1-5},
  keywords={Image color analysis;Histograms;Feature extraction;Image edge detection;Search methods;Transforms},
  doi={10.1109/IST.2017.8261544}
}

@inproceedings{montazzolli2017detection,
  author={Montazzolli, Sérgio and Jung, Claudio},
  booktitle={2017 30th SIBGRAPI Conference on Graphics, Patterns and Images (SIBGRAPI)}, 
  title={Real-Time Brazilian License Plate Detection and Recognition Using Deep Convolutional Neural Networks}, 
  year={2017},
  volume={},
  number={},
  pages={55-62},
  keywords={License plate recognition;Automobiles;Character recognition;Cameras;Databases;Training},
  doi={10.1109/SIBGRAPI.2017.14}
}

@inproceedings{corovic2018detection,
  author={Ćorović, Aleksa and Ilić, Velibor and Ðurić, Siniša and Marijan, Mališa and Pavković, Bogdan},
  booktitle={2018 26th Telecommunications Forum (TELFOR)}, 
  title={The Real-Time Detection of Traffic Participants Using YOLO Algorithm}, 
  year={2018},
  volume={},
  number={},
  pages={1-4},
  keywords={Neural networks;Object detection;Training;Real-time systems;Software algorithms;Cameras;Machine learning algorithms;Advanced Driver Assistance Systems (ADAS);Convolutional Neural Networks;Deep Learning;Machine Learning;Object Detection;YOLO Algorithm},
  doi={10.1109/TELFOR.2018.8611986}
}

@inproceedings{liu2018detection,
  author={Liu, Chengji and Tao, Yufan and Liang, Jiawei and Li, Kai and Chen, Yihang},
  booktitle={2018 IEEE 4th Information Technology and Mechatronics Engineering Conference (ITOEC)}, 
  title={Object Detection Based on YOLO Network}, 
  year={2018},
  volume={},
  number={},
  pages={799-803},
  keywords={Standards;Degradation;Training;Object detection;Data models;Neural networks;Classification algorithms;YOLO network;image processing;object detection},
  doi={10.1109/ITOEC.2018.8740604}
}

@inproceedings{laroca2018robust,
  title = {A Robust Real-Time Automatic License Plate Recognition Based on the {YOLO} Detector},
  author = {R. {Laroca} and E. {Severo} and L. A. {Zanlorensi} and L. S. {Oliveira} and G. R. {Gon{\c{c}}alves} and W. R. {Schwartz} and D. {Menotti}},
  year = {2018},
  month = {July},
  booktitle = {International Joint Conference on Neural Networks (IJCNN)},
  volume = {},
  number = {},
  pages = {1-10},
  doi = {10.1109/IJCNN.2018.8489629},
  issn = {2161-4407},
  keywords = {Cameras;Automobiles;Motorcycles;Character recognition;Object detection;Real-time systems;Licenses}
}

@inproceedings{howard2019mobilenetv3,
    author = {Howard, Andrew and Sandler, Mark and Chu, Grace and Chen, Liang-Chieh and Chen, Bo and Tan, Mingxing and Wang, Weijun and Zhu, Yukun and Pang, Ruoming and Vasudevan, Vijay and Le, Quoc V. and Adam, Hartwig},
    title = {Searching for MobileNetV3},
    booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
    month = {October},
    year = {2019}
} 

@inproceedings{wang2021transformer,
  author={Wang, Yingjin and Wang, Chuanming and Zheng, Yuchao and Fu, Huiyuan and Ma, Huadong},
  booktitle={2021 IEEE 4th International Conference on Multimedia Information Processing and Retrieval (MIPR)}, 
  title={Transformer based Neural Network for Fine-Grained Classification of Vehicle Color}, 
  year={2021},
  volume={},
  number={},
  pages={118-124},
  keywords={Adaptation models;Image color analysis;Neural networks;Lighting;Training data;Transformers;Labeling;Vehicle color recognition;Transformer;Self-attention;convolutional neural network},
  doi={10.1109/MIPR51284.2021.00025}
}

@inproceedings{kuhn2021brcars,
  author={Kuhn, Daniel M. and Moreira, Viviane P.},
  booktitle={2021 34th SIBGRAPI Conference on Graphics, Patterns and Images (SIBGRAPI)}, 
  title={BRCars: a Dataset for Fine-Grained Classification of Car Images}, 
  year={2021},
  volume={},
  number={},
  pages={231-238},
  keywords={Deep learning;Visualization;Computer vision;Computational modeling;Pipelines;Neural networks;Automobiles;fine grained computer vision;car model classification},
  doi={10.1109/SIBGRAPI54419.2021.00039}
}


@inproceedings{laroca2022cross,
  title = {On the Cross-Dataset Generalization in License Plate Recognition},
  author = {R. {Laroca} and E. V. {Cardoso} and D. R. {Lucio} and V. {Estevam} and D. {Menotti}},
  year = {2022},
  month = {Feb},
  booktitle = {International Conference on Computer Vision Theory and Applications (VISAPP)},
  volume = {},
  number = {},
  pages = {166-178},
  doi = {10.5220/0010846800003124},
  isbn = {978-989-758-555-5},
  issn = {2184-4321}
}

@misc{openalpr_br,
  title = {{OpenALPR-BR dataset}},
  author = {{OpenALPR}},
  year = {2016},
  howpublished = {\url{https://github.com/openalpr/benchmarks/tree/master/endtoend/br/}}
}

@misc{brasil2008transito,
    title = {{Resolução nº 292, de 29 de Agosto de 2008}},
    author = {{Brasil}},
    year = {2008},
    howpublished = {\url{https://www.gov.br/infraestrutura/pt-br/assuntos/transito/conteudo-contran/resolucoes/cons292.pdf}}
}

@misc{kingma2017adam,
      title={Adam: A Method for Stochastic Optimization}, 
      author={Diederik P. Kingma and Jimmy Ba},
      year={2017},
      eprint={1412.6980},
      archivePrefix={arXiv}
}

@misc{tan2021efficientnetv2,
      title={EfficientNetV2: Smaller Models and Faster Training}, 
      author={Mingxing Tan and Quoc V. Le},
      year={2021},
      eprint={2104.00298},
      archivePrefix={arXiv}
}

@misc{dosovitskiy2021vit,
      title={An Image is Worth 16x16 Words: Transformers for Image Recognition at Scale}, 
      author={Alexey Dosovitskiy and others},
      year={2021},
      eprint={2010.11929},
      archivePrefix={arXiv}
}

@misc{axalta2022global,
  title = {{Global Automotive 2022 Color Popularity Report}},
  author = {{Axalta Coating Systems}},
  year = {2022},
  howpublished = {\url{https://www.axalta.com/refinisheurope_eu/en_GB/about-axalta/colour-popularity-report-axalta.html}}
}


@misc{farias2023colorido,
  title = {{Por que o carro colorido sumiu? 67\% dos veículos no Brasil são brancos, pretos ou cinzas}},
  author = {{Victor Farias and Gabriel Croquer}},
  year = {2023},
  howpublished = {\url{https://g1.globo.com/economia/noticia/2023/08/20/por-que-o-carro-colorido-sumiu-67percent-dos-veiculos-no-brasil-sao-brancos-pretos-ou-cinzas.ghtml}}
}

@misc{harley2023cores,
  title = {{Estudo revela as cores mais populares e quais aumentam valor de revenda}},
  author = {{Michael Harley}},
  year = {2023},
  howpublished = {\url{https://forbes.com.br/forbeslife/forbes-motors/2023/10/estudo-revela-as-cores-mais-populares-e-quais-aumentam-valor-de-revenda/}}
}
